Constructive Discrepancy Minimization with Hereditary L2 Guarantees

In discrepancy minimization problems, we are given a family of sets $\mathcal{S} = \{S_1,\dots,S_m\}$, with each $S_i \in \mathcal{S}$ a subset of some universe $U = \{u_1,\dots,u_n\}$ of $n$ elements. The goal is to find a coloring $\chi : U \to \{-1,+1\}$ of the elements of $U$ such that each set $S \in \mathcal{S}$ is colored as evenly as possible. Two classic measures of discrepancy are $\ell_\infty$-discrepancy defined as $\textrm{disc}_\infty(\mathcal{S},\chi):=\max_{S \in \mathcal{S}} | \sum_{u_i \in S} \chi(u_i) |$ and $\ell_2$-discrepancy defined as $\textrm{disc}_2(\mathcal{S},\chi):=\sqrt{(1/|\mathcal{S}|)\sum_{S \in \mathcal{S}} \left(\sum_{u_i \in S}\chi(u_i)\right)^2}$. Breakthrough work by Bansal gave a polynomial time algorithm, based on rounding an SDP, for finding a coloring $\chi$ such that $\textrm{disc}_\infty(\mathcal{S},\chi) = O(\lg n \cdot \textrm{herdisc}_\infty(\mathcal{S}))$ where $\textrm{herdisc}_\infty(\mathcal{S})$ is the hereditary $\ell_\infty$-discrepancy of $\mathcal{S}$. We complement his work by giving a simple $O((m+n)n^2)$ time algorithm for finding a coloring $\chi$ such $\textrm{disc}_2(\mathcal{S},\chi) = O(\sqrt{\lg n} \cdot \textrm{herdisc}_2(\mathcal{S}))$ where $\textrm{herdisc}_2(\mathcal{S})$ is the hereditary $\ell_2$-discrepancy of $\mathcal{S}$. Interestingly, our algorithm avoids solving an SDP and instead relies on computing eigendecompositions of matrices. Moreover, we use our ideas to speed up the Edge-Walk algorithm by Lovett and Meka [SICOMP'15]. To prove that our algorithm has the claimed guarantees, we show new inequalities relating $\textrm{herdisc}_\infty$ and $\textrm{herdisc}_2$ to the eigenvalues of the matrix corresponding to $\mathcal{S}$. Our inequalities improve over previous work by Chazelle and Lvov, and by Matousek et al. Finally, we also implement our algorithm and show that it far outperforms random sampling.

==> l2algorithm.tex <==
\section{Discrepancy Minimization with Hereditary $\ell_2$ Guarantees}
\label{sec:algo}
This section gives our new algorithm for discrepancy minimization. The
goal is to prove the following:

\begin{customthm}{\ref{thm:algo}}
There is an $\tilde{O}(mn^2 + n^5)$ time algorithm that given an $m
\times n$ matrix $A$, computes a coloring $x \in \{-1,+1\}^n$
satisfying $\disctwo(A,x) = O(\sqrt{\lg n} \herdisctwo(A))$.
\end{customthm}

Our algorithm is inspired mainly by the Edge-Walk algorithm by Lovett and
Meka~\cite{lovett}. The general setup is that we first give a procedure for
partial coloring. This procedure takes a matrix $A$ and a partial
coloring $x \in [-1, + 1]^n$. We say that coordinates $i$ of $x$ such
that $|x_i| < 1-\delta$ are \emph{live}. If there are $k$ live
coordinates prior to calling the partial coloring method, then upon
termination we get a vector $\gamma$ such that the number of live
coordinates in $\hat{x} = x + \gamma$ is no more than $k/2$. At the
same time, all coordinates of $\hat{x}$ are bounded by $1$ in absolute
value and $\|A\hat{x}\|_2$ is not much larger than $\|A x\|_2$.

We start by presenting the partial coloring algorithm and then show
how to use it to get the final coloring.

\subsection{Partial Coloring}
In this section, we present our partial coloring algorithm. The algorithm takes as input an $m \times n$ matrix $A$, a
parameter $\delta > 0$ and a vector $x \in [-1 ,+1]^n$. We think of
the vector $x$ as a partial coloring and let $k$ denote the number of
live coordinates. Upon termination, it returns another vector $\gamma \in \R^n$. If we let $\hat{x} = x+ \gamma$, then we say that the algorithm \emph{succeeds} if the following holds:
\begin{itemize}
\item There are at most $k/2$ live coordinates in $\hat{x}$.
\item For all $i$, we have $|\hat{x}_i| \leq 1$.
\item $\|A\hat{x}\|_2^2-\|Ax\|_2^2\leq 2^{21} m (\herdisctwo(A))^2$.
\end{itemize}
Thus if the partial coloring algorithm succeeds, then $\|A\hat{x}\|_2$
doesn't change by much. In particular the change is related to the
hereditary $\ell_2$-discrepancy of $A$.

The main idea in our algorithm is to use the connection between
eigenvalues and hereditary $\ell_2$-discrepancy that we proved in
Corollary~\ref{thm:l2eigen}. Our algorithm proceeds in iterations,
where in each step it samples a random vector $v$ that it adds to a
result vector $\gamma$. The way we sample $v$ is roughly to find the 
eigenvectors of $A^TA$ and then sample $v$ orthogonal to the
eigenvectors corresponding to the largest eigenvalues. This bounds the
difference $\|A(x + \gamma)\|_2 - \|A(x+\gamma+v)\|_2$. in terms of
the eigenvalues and thus hereditary $\ell_2$-discrepancy. At the same time, we use the ideas by Lovett
and Meka where we include constraints forcing $v$ orthogonal to $e_i$
for every coordinate $i$ that is not live. Finally, if the vectors we
sample are ``short'' enough, the coordinates of $x + \gamma$ will
never exceed $1$ with good probability. The full details of the algorithm are as follows:

\paragraph{PartialColor($A$, $x$, $\delta$):}
\begin{enumerate}
\item Let $k$ denote the number of live coordinates in $x$.
\item Initialize $\gamma \gets \zero$, $\eps \gets \delta/\sqrt{c_0
  \lg(k/\delta)}$ for a big enough constant $c_0$, $T \gets 160
\eps^{-2}$.
\item Let $C$ denote the $m \times n$ matrix obtained from $A$ by
  zeroing all columns corresponding to coordinates that are not live.
\item Compute an eigendecomposition of $C^TC$ to obtain the
  eigenvalues $\lambda_1 \geq \cdots \geq \lambda_n \geq 0$ and corresponding eigenvectors $\mu_1,\dots,\mu_n$.
\item For $j=1,\dots,T$:
\begin{enumerate}
\item Compute the set $S$ of coordinates $i$ such that $|(x + \gamma)_i| \geq 1-\delta$. If $|S| \geq n-k/2$, return $\gamma$.
\item Form an $n \times (|S|+k/4)$ matrix $B$ having $\mu_1,\dots,\mu_{k/4}$ as columns, as well as $e_j$ for every $j \in S$.
\item Compute a QR-factorization $B = QR$ of $B$. The last $k/4$ columns $q_{n-k/4 + 1},\dots, q_n$ of $Q$ form an orthonormal basis of a $k/4$-dimensional subspace $V$ orthogonal to the span of $\mu_1,\dots,\mu_{k/4}$ and all $e_j$ with $j \in S$.
\item Let $g_{n-k/4 + 1},\dots,g_n$ be independent $\Norm(0,1)$ random variables and set $v := (\sum_{i=n-k/4 + 1}^n g_i q_i)$.
\item Update $\gamma \gets \gamma + \eps v$.
\end{enumerate}
\item Abort.
\end{enumerate}

If the algorithm terminates in the abort step, we also say that it does not
succeed. Our goal is to prove the following about our partial coloring algorithm:

\begin{lemma}
\label{lem:partial}
Given a parameter $0 < \delta < 1$ and an $m \times n$ matrix $A$ and
a vector $x \in [-1, + 1]$, the
\textbf{PartialColor} algorithm runs in time $O(mn^2 +
n^3\delta^{-2}\lg(n/\delta))$ and succeeds with probability at least $1/8$.
\end{lemma}

The bound on the running time is shown as follows: Computing $C^TC$
takes $O(mn^2)$ time. Computing an eigendecomposition of $C^TC$ takes time
$O(n^3)$. The running time of an iteration of the for-loop is
dominated by the time to compute a QR-factorization, which takes
$O(n^3)$ time. Since the loop runs $T = O(\eps^{-2}) = O(\delta^{-2}
\lg(n/\delta))$ times, the running time follows.

What remains is to prove the claimed success probability. We split the
proof into three steps, arguing that each of the three requirements
for succeeding are satisfied with high probability. At the end, we can
simply apply a union bound.

Due to space constraints, we prove the following results in the
appendix:
\begin{lemma}
\label{lem:smallmax}
The \textbf{PartialColor} algorithm satisfies that:
$$\Pr[\max_i |\hat{x}_i| > 1]  = k^{-\Omega(1)}.$$
\end{lemma}

\begin{lemma}
\label{lem:fewlive}
The \textbf{PartialColor} algorithm satisfies that there are no more
than $k/2$ live coordinates in $\hat{x} = x+\gamma$ with probability
at least $7/8$.
\end{lemma}

The proof of the above two follows previous work quite closely, so we
have chosen to present the proof that the discrepancy changes by
little upon updating $x$ to $\hat{x} = x + \gamma$.

\paragraph{Growth in Discrepancy.}
In this paragraph, we bound the increase in discrepancy when updating
$x$ to $\hat{x} = x + \gamma$. We start
by defining a few random variables that we will need throughout our
proofs. Let $Q_{j,n-k/4+1},\dots,Q_{j,n}$ be the random variables giving the
vectors $q_{n-k/4+1},\dots,q_n$ computed in step (c) of the above
algorithm during the $j$'th iteration of the for-loop. If the
algorithm already terminated in step (a) in the $j$'th iteration or
earlier, we
let each $Q_{j,i}$ equal $\zero$. Let
$G_{j,n-k/4+1},\dots,G_{j,n}$ be the random variables giving the values
$g_{n-k/4+1},\dots,g_n$ sampled in step (d) during the $j$'th iteration
of the for-loop (taking values $0$ if we don't reach the $j$'th iteration). Finally, let $V_j$ be the random variable giving the vector $v$ computed in the
$j$'th iteration of the for-loop, i.e. $V_j = \sum_{i=n-k/4+1}^n G_{j,i}
Q_{j,i}$.

Since we are dealing with $\mathcal{N}(0,1)$ distributed random
variables, the following tail bound will be useful:
\begin{fact}
If $X$ is $\mathcal{N}(0,1)$ distributed, then $\Pr[|X| \geq \lambda]
\leq 2 \exp(\lambda^2/2)$.
\end{fact}
We will also need the following facts about normal distributed random variables:
\begin{fact}
If $X \sim \mathcal{N}(0,\sigma_x^2)$ and $Y \sim
\mathcal{N}(0,\sigma_y^2)$ with $X$ and $Y$ independent, then $aX + bY
\sim \mathcal{N}(0,a^2\sigma_x^2 + b^2\sigma_y^2)$ if $a$ and $b$ are
constants. We also have $\E[X^2] = \sigma_x^2$.
\end{fact}

We are ready to bound the discrepancy increase when changing $x$ to $\hat{x} = x + \gamma$ For this, we first rewrite
$\|A(\gamma+x)\|_2^2-\|Ax\|_2^2$. 
We see that:
\begin{eqnarray*}
\|A(\gamma+x)\|_2^2-\|Ax\|_2^2 = 
\|A\gamma\|_2^2 + \|Ax\|_2^2 + 2\gamma^TA^TAx - \|Ax\|_2^2 = 
\|A\gamma\|_2^2 + 2\gamma^TA^TAx.
\end{eqnarray*}
We start by examining $\|A\gamma\|_2^2$ and see that:
\begin{eqnarray*}
\E\left[ \|A \gamma \|_2^2 \right] =
\eps^2 \E\left[ \|\sum_j AV_j \|_2^2 \right] =
\eps^2 \sum_j \sum_h \E\left[  V_h^TA^TA V_j \right].
\end{eqnarray*}
Consider first a pair $j \neq h$ and assume wlog. $h > j$. Then $V_h^TA^TA V_j = \langle V_h,
A^TAV_j \rangle$. Now for every value $v \in \supp(V_j)$, we see that
the distribution of $\langle V_h,
A^TAV_j \rangle$ is symmetric around $0$ conditioned on $V_j =
v$. Thus $\E\left[  V_h^TA^TA V_j \right]=0$. Therefore
\begin{eqnarray*}
\E\left[ \|A \gamma \|_2^2 \right] &=&
\eps^2 \sum_j \E\left[  V_j^TA^TA V_j \right].
\end{eqnarray*}
By construction, we know that $V_j$ is orthogonal to the eigenvectors
$\mu_1,\dots,\mu_{k/4}$ of $C^TC$. Furthermore, $V_j$ is orthogonal to
every $e_i$ where $i$ was not live when we started the partial
coloring. Thus $V_j^TA^TA V_j = V_j^TC^TCV_j$ and hence $V_j^TA^TA V_j \leq \lambda_{k/4}
\|V_j\|_2^2$. We continue:
\begin{eqnarray*}
\E\left[ \|A \gamma \|_2^2 \right] &\leq& \eps^{2}\lambda_{k/4}
\sum_j \E\left[ \|V_j\|_2^2 \right] \\
&=&   \eps^{2}\lambda_{k/4}
\sum_j \sum_{i=n-k/4+1}^n \E\left[ G_{j,i}^2 \right] \\
&\leq& \eps^{2}\lambda_{k/4} T k/4 
= 40 k \lambda_{k/4}.
\end{eqnarray*}
Thus by Markov's inequality, $\Pr[ \|A \gamma \|_2^2 > 320 k
\lambda_{k/4}] \leq 1/8$. Consider now $\E[\gamma^TA^TAx]$:
\begin{eqnarray*}
\E[\gamma^TA^TAx] &=& \sum_{j=1}^T \E[\langle \eps V_j, A^TAx \rangle].
\end{eqnarray*}
Since $A^TAx$ is just a fixed vector, we have that the distribution of
$\langle \eps V_j,
A^TAx \rangle$ is symmetric around $0$ and hence $\Pr[\gamma^TA^TAx
\leq 0] \geq 1/2$. By Markov's inequality and a union bound, we
simultaneously have that $\|A \gamma\|_2^2 \leq 320 k\lambda_{k/4}$ and $\gamma^TA^TAx
\leq 0$ with probability at least $1-1/8-1/2 =3/8$. Since
$$
\|A(\gamma+x)\|_2^2-\|Ax\|_2^2 = \|A \gamma\|_2^2 + 2\gamma^TA^TAx
$$
we conclude that with probability at least $3/8$, we have 
$$
\|A(\gamma+x)\|_2^2-\|Ax\|_2^2 \leq 320 k\lambda_{k/4}.
$$
We would like to use Corollary~\ref{thm:l2eigen} to relate $k
\lambda_{k/4}$ to the hereditary discrepancy of $A$. Unfortunately,
$C$ is $m \times n$ and we would lose something like a $\sqrt{n/k}$
factor, which is quite terrible as $k$ decreases. Our key idea is to
relate $\lambda_{k/4}$ to the eigenvalues of an $m \times k$ submatrix
of $A$ and then use that the hereditary discrepancy of such a
submatrix is less than or equal to the hereditary discrepancy of $A$.

So consider the $m \times k$ matrix $D$ obtained from $C$ by deleting
the columns that were zeroed out (i.e. $D$ is the submatrix obtained
from $A$ by deleting all columns corresponding to coordinates that
were not live when we started the partial coloring). Let $\lambda'_1
\geq \cdots \geq \lambda'_k \geq 0$ denote the eigenvalues of $D^TD$. We
claim $\lambda'_j = \lambda_j$ for all $j$. To see this, observe that
if $\lambda_j > 0$, then we must have that $\mu_j$ has all coordinates
$i$ corresponding to zeroed columns in $C$ equal to $0$ as otherwise
we cannot have $\mu_j = \lambda_j C^TC\mu_j$ (if the $i$'th column of $C$ is
zeroed, so is the $i$'th row of $C^TC$). This means that if we take
$\mu_j$ and delete all coordinates corresponding to zeroed out columns
of $C$, then the resulting vector $\mu'_j$ satisfies $\mu'_j =
\lambda_j D^TD \mu'_j$, thus all $\mu'_j$ are also distinct
eigenvectors of $D^TD$ having the corresponding eigenvalues
$\lambda_j$. In the opposite direction, if $\mu$ is an
eigenvector of $D^TD$ with non-zero eigenvalue $\lambda$, then if we pad with
zeroes corresponding to the columns deleted when going from $C$ to
$D$, we would also get an eigenvector for $C^TC$ with the same
non-zero eigenvalue. Hence $D^TD$ and $C^TC$ have exactly the same non-zero
eigenvalues. It therefore holds with probability at least $3/8$ that:
$$
\|A(\gamma+x)\|_2^2-\|Ax\|_2^2 \leq 320 k\lambda'_{k/4}.
$$
Now $D$ is an $m \times k$ matrix. Thus it follows from
Corollary~\ref{thm:l2eigen} that 
\begin{eqnarray*}
320 k\lambda'_{k/4} = 320 \cdot 2^{7} e^2 \pi m \cdot
\frac{(k/4)^2}{e^2}\frac{\lambda'_{k/4}}{8 \pi m k} 
 \leq 2^{16} e^2 \pi m (\herdisctwo(D))^2.
\end{eqnarray*}
But $D$ was obtained by deleting columns of $A$ and thus
$\herdisctwo(D) \leq \herdisctwo(A)$ by definition, and we get that with probability
at least $3/8$, we have:
$$
\|A(\gamma+x)\|_2^2-\|Ax\|_2^2 \leq 2^{16} e^2 \pi m (\herdisctwo(A))^2
\leq 2^{21}  m (\herdisctwo(A))^2.
$$
Using a union bound together with Lemma~\ref{lem:smallmax} and
Lemma~\ref{lem:fewlive} completes the proof of Lemma~\ref{lem:partial}.

\subsection{The Final Algorithm}
Now that we have the \textbf{PartialColor} algorithm, getting to a
lower discrepancy coloring is straight forward. Given an $m \times n$
matrix $A$, we initialize $x \gets \zero$. We then repeatedly invoke
\textbf{PartialColor}($A$, $x$, $\delta$) for some parameter
$\delta>0$ to be fixed shortly. Each call returns a vector
$\gamma$. If the call to \textbf{PartialColor} succeeds, we update $x
\gets x + \gamma$ and continue. Otherwise, we discard $\gamma$ and try
again. Since \textbf{PartialColor} succeeds with constant probability,
we expect to discard $\gamma$ only a constant number of times. We stop
once there are no live coordinates in $x$, i.e. all coordinates
satisfy $1-\delta \leq |x_i| \leq 1$.

In each iteration, the number of live coordinates of $i$ decreases by
at least a factor two, and thus we are done after at most $\lg n$
iterations. This means that the final vector $x$ satisfies
\begin{eqnarray*}
\|Ax\|_2^2 &\leq& \lg n (2^{21} m (\herdisctwo(A))^2)
\Rightarrow \\
\|Ax\|_2 &=& O(\sqrt{m \lg n} \herdisctwo(A)).
\end{eqnarray*}
We now round each coordinate to the nearest of $1$ and $-1$ to obtain
a coloring $\hat{x} \in \{-1,+1\}^n$. Let $\lambda_1 \geq \cdots \geq
\lambda_n \geq 1$ be the eigenvalues of $A^TA$. Since $\|\hat{x}-x\|_\infty \leq
\delta$, we have
\begin{eqnarray*}
\|A(\hat{x}-x)\|_2 \leq \sqrt{\lambda_1}\|\hat{x}-x\|_2 \leq \sqrt{\lambda_1}\delta \sqrt{n}.
\end{eqnarray*}
From Corollary~\ref{thm:l2eigen}, we get that $\sqrt{\lambda_1} =
O(\herdisctwo(A) \sqrt{mn})$. Thus $\sqrt{\lambda_1}\delta \sqrt{n} =
O(n \delta \sqrt{m} \herdisctwo(A))$. We now fix $\delta = 1/n$ and
get $\sqrt{\lambda_1}\delta \sqrt{n} = O(\sqrt{m} \herdisctwo(A))$. We
then conclude:
\begin{eqnarray*}
\disctwo(A,\hat{x}) = (1/\sqrt{m})\|A\hat{x}\|_2 
\leq  (1/\sqrt{m})(\|Ax\|_2 + \|A(\hat{x}-x)\|_2) 
= O(\sqrt{\lg n}
\cdot \herdisctwo(A)).
\end{eqnarray*}
Since the running time of \textbf{PartialColor} is $O(mn^2 +
n^3\delta^{-2}\lg(n/\delta))$ and we call it an expected $O(\lg n)$
times with $\delta=1/n$, the
final algorithm has an expected running time of $\tilde{O}(mn^2 +
n^5)$. This concludes the proof of Theorem~\ref{thm:algo}.



==> prelim.tex <==
\section{Preliminaries}

\begin{definition}
Let $A$ be an $m \times n$ real matrix. Then its $\ell_\infty$-discrepancy
is defined as:
$$
\disc(A) := \min_{x \in \{-1,+1\}^n} \|Ax\|_\infty.
$$
\end{definition}

\begin{definition}
Let $A$ be an $m \times n$ real matrix and $x \in \{-1,+1\}^n$. Then
the $\ell_2$-discrepancy of $A$ wrt. $x$ is
$$
\disctwo(A,x) := \frac{1}{\sqrt{m}}\|Ax\|_2.
$$
The $\ell_2$-discrepancy of $A$ is defined as:
$$
\disctwo(A) := \min_{x \in \{-1,+1\}^n} \disctwo(A,x).
$$
\end{definition}

\begin{definition}
Let $A$ be an $m \times n$ real matrix. Then its hereditary
$\ell_\infty$-discrepancy is defined as:
$$
\herdisctwo(A) := \max_B \disc(B),
$$
where $B$ ranges over all matrices obtained by removing a subset of
the columns in $A$.
\end{definition}

\begin{definition}
Let $A$ be an $m \times n$ real matrix. Then its hereditary
$\ell_2$-discrepancy is defined as:
$$
\herdisctwo(A) := \max_B \disctwo(B),
$$
where $B$ ranges over all matrices obtained by removing a subset of
the columns in $A$.
\end{definition}

\begin{definition}
Let $A$ be an $m \times n$ real matrix. Then its linear $\ell_\infty$-discrepancy
is defined as:
$$
\lindisc(A) := \max_{c \in [-1,+1]} \min_{x \in \{-1,+1\}^n} \|A(x-c)\|_\infty.
$$
\end{definition}
